Performance Analysis of ISAC Slicing with Sensing-Assisted Communication and Communication-Assisted Sensing

Integrated Sensing and Communication (ISAC) will allow 6G networks to provide both sensing and communication services through shared infrastructure and spectrum resources. However, network slicing that views these services as distinct slices with distinct objectives and performance requirements will inevitably miss the emergent value of integrating them. By considering Sensing-Assisted Communication (SAC) and Communication-Assisted Sensing (CAS), which create interdependencies between services, we can observe trade-offs in resources dimensioned to support each slice and, ultimately, the ISAC slicing performance. As such, this paper proposes a performance analysis of an ISAC slicing framework that accounts for resource allocation and sensor density, as well as SAC and CAS, dimensioned to achieve slice-specific Service-Level Agreement (SLA) satisfaction. Numerical simulations, across different bandwidth allocations, sensor deployments, and demand scenarios, show that ISAC slicing performance is fundamentally constrained by sensing resolution, shaped by demand, and scaled by sensor deployment. These findings provide insights for the design of future ISAC slicing mechanisms.

==> acronyms.tex <==
\DeclareAcronym{SLA}{
    short=SLA,
    long=Service Level Agreement
}

\DeclareAcronym{RBG}{
    short=RBG,
    long=Resource Block Group
}

\DeclareAcronym{UE}{
    short=UE,
    long=User Equipment
}

\DeclareAcronym{BS}{
    short=BS,
    long=Base Station
}

\DeclareAcronym{SLAd}{
    short=SLAd,
    long=\ac{SLA}-drift
}

\DeclareAcronym{IAB}{
    short=IAB,
    long=Integrated Access Backhaul
}

\DeclareAcronym{TTI}{
    short=TTI,
    long=Transmission Time Interval
}

\DeclareAcronym{QoS}{
    short=QoS,
    long=Quality of Service
}

\DeclareAcronym{UPF}{
    short=UPF,
    long=User Plane Function
}

\DeclareAcronym{LTT}{
    short=LTT,
    long=Long-Term Throughput
}

\DeclareAcronym{CT}{
    short=CT,
    long=Constant Throughput
}

\DeclareAcronym{EWMA}{
    short=EWMA,
    long=Exponential Weight Moving Average
}

\DeclareAcronym{PF}{
    short=PF,
    long=Proportional Fairness
}

\DeclareAcronym{MT}{
    short=MT,
    long=Maximum Throughput
}

\DeclareAcronym{5QI}{
    short=5QI,
    long=5G Quality Indicator
}


\DeclareAcronym{3GPP}{
    short=3GPP,
    long=3rd Generation Partnership Project
}

\DeclareAcronym{GBR}{
    short=GBR,
    long=Guaranteed Bit Rate
}

\DeclareAcronym{DC-GBR}{
    short=DC-GBR,
    long=Delay-Critical \ac{GBR}
}

\DeclareAcronym{Non-GBR}{
    short=Non-GBR,
    long=Non-\ac{GBR}
}

\DeclareAcronym{PDB}{
    short=PDB,
    long=Packet Delay Budget
}

\DeclareAcronym{HOB}{
    short=HOB,
    long=Head-of-Buffer
}

\DeclareAcronym{RAN}{
    short=RAN,
    long=Radio Access Network
}

\DeclareAcronym{O-RAN}{
    short=O-RAN,
    long=Open-\ac{RAN}
}

\DeclareAcronym{RRM}{
    short=RRM,
    long=Radio Resource Management
}

\DeclareAcronym{RIC}{
    short=RIC,
    long=\ac{RAN} Intelligent Controller
}

\DeclareAcronym{Near-RT RIC}{
    short=Near-RT RIC,
    long=Near-Real-Time \ac{RIC}
}

\DeclareAcronym{enD}{
    short=enD,
    long=enhanced \ac{DREAMIN}
}

\DeclareAcronym{DREAMIN}{
    short=DREAMIN,
    long=Drift and REsource Allocation Minimization 
}

\DeclareAcronym{RL}{
    short=RL,
    long=Reinforcement Learning
}

\DeclareAcronym{MAC}{
    short=MAC,
    long=Medium Access Control
}

\DeclareAcronym{O-DU}{
    short=O-DU,
    long=Open-\ac{DU}
}

\DeclareAcronym{DU}{
    short=DU,
    long=Distributed Unit
}

\DeclareAcronym{Non-RT RIC}{
    short=Non-RT RIC,
    long=Non-Real-Time \ac{RIC}
}

\DeclareAcronym{SMO}{
    short=SMO,
    long=Service Management and Orchestration
}

\DeclareAcronym{V2X}{
    short=V2X,
    long=Vehicle-to-Everything
}

\DeclareAcronym{KPM}{
    short=KPM,
    long=Key Performance Metric
}

\DeclareAcronym{RS}{
    short=RS,
    long=Reference Signal
}

\DeclareAcronym{SaaS}{
    short=SaaS,
    long=Sensing as a Service
}

\DeclareAcronym{CaaS}{
    short=CaaS,
    long=Communication as a Service
}

\DeclareAcronym{ISAC}{
    short=ISAC,
    long=Integrated Sensing and Communication,
    short-indefinite = an, 
    long-indefinite  = an 
}

\DeclareAcronym{PRB}{
    short=PRB,
    long=Physical Resource Block
}


\DeclareAcronym{RoI}{
    short=RoI,
    long=Region of Interest,
}

\DeclareAcronym{eMBB}{
    short=eMBB,
    long=enhanced Mobile Broadband,
}

\DeclareAcronym{URLLC}{
    short=URLLC,
    long=Ultra-Reliable Low-Latency Communication,
}

\DeclareAcronym{mMTC}{
    short=mMTC,
    long=massive Machine-Type Communication,
}

\DeclareAcronym{XaaS}{
    short=XaaS,
    long=Everything as a Service,
}

\DeclareAcronym{MCS}{
    short=MCS,
    long=Modulation and Conding Scheme,
}

\DeclareAcronym{CSI-RS}{
    short=CSI-RS,
    long=Channel State Information \ac{RS},
}

\DeclareAcronym{gNB}{
    short=gNB,
    long=Next Generation Node B,
}

\DeclareAcronym{SNR}{
    short=SNR,
    long=Signal-to-Noise Ratio
}

\DeclareAcronym{LABORA}{
    short=LABORA,
    long=Computer Networks and Distributed Systems LABORAtory
}

\DeclareAcronym{CCI}{
    short=CCI,
    long=Commonwealth Cyber Initiative
}


\DeclareAcronym{CRLB}{
    short=CRLB,
    long=Cramér-Rao Lower Bound
}

\DeclareAcronym{LOS}{
    short=LOS,
    long=Line of Sight
}

\DeclareAcronym{RCS}{
    short=RCS,
    long=Radar Cross-Section
}

\DeclareAcronym{OFDM}{
    short=OFDM,
    long=Orthogonal Frequency-Division Multiplexing
}

\DeclareAcronym{ULA}{
    short=ULA,
    long=Uniform Linear Array,
    short-indefinite = a, 
    long-indefinite  = a 
}

\DeclareAcronym{HPBW}{
    short=HPBW,
    long=Half-Power Beamwidth
}

\DeclareAcronym{FDD}{
    short=FDD,
    long=Frequency Division Duplexing
}

\DeclareAcronym{PRS}{
    short=PRS,
    long=Positioning Reference Signal
}

\DeclareAcronym{SSR}{
    short=SSR,
    long=\ac{SLA} Satisfaction Rate
}

\DeclareAcronym{DL}{
    short=DL,
    long=Downlink
}


\DeclareAcronym{SAC}{
    short=SAC,
    long=Sensing-Assisted Communication
}

\DeclareAcronym{CAS}{
    short=CAS,
    long=Communication-Assisted Sensing
}

\DeclareAcronym{CPI}{
    short=CPI,
    long=Coherent Processing Interval
}

\DeclareAcronym{UMi}{
    short=UMi,
    long=Urban Microcell
}

\DeclareAcronym{PPP}{
    short=PPP,
    long=Poisson Point Process
}

\DeclareAcronym{NSB}{
    short=NSB,
    long=Normalized Sensing Bandwidth
}

\DeclareAcronym{PP}{
    short=PP,
    short-plural=,
    long=Percentual Point
}

